Softmax Policy Gradient Methods Can Take Exponential Time to Converge

The softmax policy gradient (PG) method, which performs gradient ascent under softmax policy parameterization, is arguably one of the de facto implementations of policy optimization in modern reinforcement learning. For $\gamma$-discounted infinite-horizon tabular Markov decision processes (MDPs), remarkable progress has recently been achieved towards establishing global convergence of softmax PG methods in finding a near-optimal policy. However, prior results fall short of delineating clear dependencies of convergence rates on salient parameters such as the cardinality of the state space $\mathcal{S}$ and the effective horizon $\frac{1}{1-\gamma}$, both of which could be excessively large. In this paper, we deliver a pessimistic message regarding the iteration complexity of softmax PG methods, despite assuming access to exact gradient computation. Specifically, we demonstrate that the softmax PG method with stepsize $\eta$ can take \[ \frac{1}{\eta} |\mathcal{S}|^{2^{\Omega\big(\frac{1}{1-\gamma}\big)}} ~\text{iterations} \] to converge, even in the presence of a benign policy initialization and an initial state distribution amenable to exploration (so that the distribution mismatch coefficient is not exceedingly large). This is accomplished by characterizing the algorithmic dynamics over a carefully-constructed MDP containing only three actions. Our exponential lower bound hints at the necessity of carefully adjusting update rules or enforcing proper regularization in accelerating PG methods.

==> MDP-key-property.tex <==
\section{Some crucial properties of the constructed MDP}
\label{sec:optimal-property}

In this section, we list out a few crucial properties associated with the constructed MDP. 
First we characterize the optimal value functions as follows, whose proof can be found in Section~\ref{sec:proof-lemma:basic-properties-MDP-Vstar}.
The collection of basic relations regarding more general policies are deferred to Section~\ref{sec:preliminaries}. 


\begin{lemma}[Optimal values]
	\label{lem:basic-properties-MDP-Vstar}
	Suppose that $\gamma^{2H}\geq 2/3$ and $H\geq 2$.
	%$H\leq \frac{\log(3/2)}{2\log(1/\gamma)}$ and that $2\gamma^4>1$. 
	Then one has 
%
\begin{subequations}
\begin{align}
	V^{\star}(0)  =0,\qquad V^{\star}(s) & =Q^{\star}(s,a_1) = \gamma^{2s},\quad ~~~ 1\leq s\leq H,\\
	 \qquad\quad\, V^{\star}(\overline{s}) &=Q^{\star}(\overline{s},a_1) =\gamma^{2s+1},\quad1\leq s\leq H.
	 %\qquad\quad V^{\star}(1)  &= Q^{\star}(1,a_{1}) = \gamma^2, \\
	 %\quad\quad  s_1\in \mathcal{S}_1, \\
	 %\qquad\quad V^{\star}(2)  &= Q^{\star}(2,a_{1}) = \gamma^4, 
	 %\quad\quad  s_2\in \mathcal{S}_2,
\end{align}
\end{subequations}
%
and the optimal policy is to take action $a_1$ in all non-absorbing states. 
In addition, for any policy $\pi$ and any state-action pair $(s,a)$, one has $Q^{\pi}(s,a) \geq - \gamma^2$.
\end{lemma}
%

Lemma~\ref{lem:basic-properties-MDP-Vstar} tells us that for the constructed MDP, the optimal policy at all primary states takes a simple form: one only needs to stick to action $a_{1}$. 
When $\gamma \approx 1$ and $\gamma^H\approx 1$, Lemma~\ref{lem:basic-properties-MDP-Vstar} also  reveals that the optimal values of all non-absorbing major states are fairly close to 1, namely,  
%
\begin{align}
	V^{\star}(s)\approx 1 \qquad \text{for all } s\in \{1,\cdots, H\} \cup \{\overline{1},\cdots, \overline{H}\}.
	\label{eq:optimal-values-approx-1}
\end{align}
%
Moreover, it indicates that the Q-function  (and hence the value function) is always bounded below by $-1$. 



To investigate the number of steps needed for SPG to converge to the optimal policy, 
a family of key quantities that we shall pay particular attention to are   
the number of iterations needed for  $V^{(t)}(s)$ to surpass a prescribed threshold $\tau$ ($\tau<1$) {\em before} it reaches its optimal value. 
To be precise,  for each $s \in \{3,\cdots,H\} \cup \{\overline{1},\cdots,\overline{H}\}$ and any given threshold $\tau>0$, 
we introduce the following {\em crossing time}:
%
\begin{align}
\label{eqn:approx-optimal-time}
	t_s(\tau) := \arg\min \big\{t \mymid V^{(t)}(s) \geq \tau \big\}.	
\end{align}
%
When it comes to the buffer state subsets $\cS_1$ and $\cS_2$, we define the crossing time analogously as follows
%
\begin{align}
\label{eqn:approx-optimal-time-buffer}
	t_1(\tau) \coloneqq \arg\min \big\{t \mymid V^{(t)}(1) \geq \tau \big\}
	\qquad \text{and}\qquad 
	t_2(\tau) \coloneqq \arg\min \big\{t \mymid V^{(t)}(2) \geq \tau \big\},
\end{align}
%
where we recall the notation \eqref{eq:convenient-notation-V1-V2-Q1-Q2}. 



\paragraph{Ordering of crossing times.}
Recalling the definition \eqref{eqn:approx-optimal-time} of the crossing time $t_s(\cdot)$, we know that 
%
\begin{align}
	V^{(t)}(s) < \taun_s \qquad \text{for all }t< t_s(\taun_s),
	\label{eq:V-t-sprime-3-H-s}
\end{align}
with $\tau_{s}$ defined in expression~\eqref{defn:tau-s}. 
%
One can demonstrate (by invoking Part (v) of Lemma~\ref{lem:basic-properties-MDP-pi} recursively)
% and \eqref{eq:compare-gamma-half-tau-tau-minus} 
that: for any $2\leq s \leq H$ and any $t< t_s(\taun_s)$, we have 
%
\begin{align}
	V^{(t)}(s^{\prime})< \gamma^{1/2}\tau_{s^{\prime}} < \taun_{s^{\prime}} \qquad  \text{for all }s^{\prime}\text{ obeying }s \le s^{\prime} \leq H.
	\label{eq:V-t-sprime-3-H}
\end{align}
%
This in turn uncovers the following monotonicity property: 
%
\begin{align}
	t_2(\taun_2)\leq t_3(\taun_3)\leq  \cdots \leq t_H(\taun_H). 
	\label{eq:monotonicity-t-s-tau-s}
\end{align}




==> introduction_colt.tex <==

\section{Introduction}
 

Despite their remarkable empirical popularity in modern reinforcement learning \citep{mnih2015human,silver2016mastering},  theoretical underpinnings of policy gradient (PG) methods and their variants \citep{williams1992simple,sutton2000policy,kakade2002natural,peters2008natural,konda2000actor} remain severely obscured. Due to the nonconcave nature of value function maximization induced by complicated dynamics of the environments, it is in general highly challenging to pinpoint the computational efficacy of PG methods in finding a near-optimal policy. 
Motivated by their practical importance, a recent strand of work sought to make progress towards demystifying the effectiveness of policy gradient type methods (e.g., \citet{agarwal2019optimality,mei2020global,agarwal2019optimality,bhandari2019global,shani2019adaptive,cen2020fast,fazel2018global,zhang2020sample,zhang2020global,bhandari2020note}), focusing primarily on canonical settings such as tabular Markov decision processes (MDPs) for discrete problems and linear quadratic regulators for continuous problems. % in addition to proper policy parameterization. 

%The impacts of several important algorithmic tricks --- e.g., policy parameterization, entropy regularization, preconditioning via natural gradients --- have been investigated as well. 

%A recent surge of activities aim to demystify their effectiveness in canonical settings such as tabular Markov decision processes (MDP) for discrete problems \citep{agarwal2019optimality,mei2020global}, and linear quadratic regulators for continuous problems \citep{fazel2018global}. Landscape properties of the value function, which are important indicators to the performance of PG, are also studied \citep{bhandari2019global}.

%, despite the presence of nonconcavity and flat saddle points

The current paper studies PG methods with softmax parameterization --- commonly referred to as {\em softmax policy gradient} methods --- which are among the de facto implementations of PG methods in practice. An intriguing result was obtained by the recent work \citet{agarwal2019optimality}, which established asymptotic global convergence of softmax PG methods for infinite-horizon $\gamma$-discounted tabular MDPs. Subsequently, \citet{mei2020global} further demonstrated that softmax PG methods are capable of finding an $\epsilon$-optimal policy within $O(1/\epsilon)$ iterations (see Table~\ref{tab:comparisons} for the precise form). While these results take an important step towards understanding softmax PG methods, 
caution needs to be exercised before declaring fast convergence of the algorithm. 
In particular, the iteration complexity derived by \citet{mei2020global} falls short of delineating clear dependencies on important salient parameters of the MDP, such as the dimension of the state space and the effective horizon $1/(1-\gamma)$. These parameters are often enormous in various contemporary RL applications, and might play a pivotal role in determining the computational complexity of softmax PG methods. 


Additionally, existing literature largely concentrated on developing algorithm-dependent upper bounds on the iteration complexities. Note, however, that upper bounds on the computational complexities of distinct algorithms cannot be directly compared for benchmarking purposes in a decisive manner. As a concrete example, it is of practical interest to benchmark softmax PG methods against natural policy gradient (NPG) methods with softmax parameterization --- a variant of policy optimization lying underneath several mainstream RL algorithms such as {\em proximal policy optimization} (PPO) \citep{schulman2017proximal} and  {\em trust region policy optimization} (TRPO) \citep{schulman2015trust}. While it is tempting to claim superiority of NPG methods over softmax PG methods given the appealing convergence properties of NPG methods \citep{agarwal2019optimality} (see Table~\ref{tab:comparisons}), existing theory fell short to reach such a conclusion due to the lack of explicit and meaningful convergence lower bounds for softmax PG methods. 


%
The above considerations lead to a natural question that we aim to address in the present paper: 
%In fact, the same diagnosis applies to entropy-regularized SPG, where the iteration complexity of NPG achieves a linear convergence rate that is nearly independent of the dimension of the MDP \citep{cen2020fast}, while PG achieves a linear rate with similar unspecified dependencies with the MDP parameters \citet{mei2020global}.
\begin{center}
{\em Can we develop a lower bound on the iteration complexity of softmax PG methods that reflects explicit dependency on the salient parameters of the MDP?}
\end{center}



 
 
 %While it is tempting to conclude that NPG has a better iteration complexity than PG, it is premature to draw such a conclusion by only comparing the respective upper bounds of the algorithms under comparison. 



\subsection{Main result}

As a main contribution of this paper, we deliver a somewhat surprising message that can be described in words as follows:
%
\begin{center}
{\em Softmax PG methods can take exponential time to converge, even in the presence of a benign initialization and an initial state distribution amenable to exploration.   }
\end{center}
%
To be precise, our finding is formally stated in the following theorem. Here and throughout, $|\cS|$ denotes the size of the state space, $0<\gamma<1$ is the discount factor, $V^{\star}$ indicates the optimal value function, $\eta>0$ is the learning rate or stepsize, whereas  $V^{(t)}$ represents the value function estimate of softmax PG methods in the $t$-th iteration; see Section~\ref{sec:backgrounds} for formal descriptions. 
%
\begin{theorem} 
\label{thm:unregularized}
	Suppose  $0.96< \gamma < 1$ and $0< \eta \leq (1-\gamma)^2 / 5$. There exists an MDP such that the number of iterations needed for softmax PG methods --- which starts from a uniform policy and employs exact gradient computation over the uniform state distribution --- to reach $\| V^{\star}-V^{(t)} \|_{\infty}\leq 0.15 $ is at least
%
\begin{align} 
	\label{eq:t-bound}
	\frac{c_1}{\eta} |\cS| ^{ 2^{ \frac{c_2}{1-\gamma}}}.
\end{align}
Here, $c_1, c_2>0$ are some universal constants independent of the salient parameters of the MDP, 
	and we assume $ |\cS| \ge c_3 (1-\gamma)^{-6}$ for some universal constant $c_3>0$.
\end{theorem}
For simplicity of presentation, Theorem~\ref{thm:unregularized} is stated for the long-horizon regime where $\gamma > 0.96$; it continues to hold when $\gamma > c_0$ for some smaller constant $c_0>0$.
Our result is obtained based on constructing a hard MDP instance --- which is a properly augmented chain-like MDP --- for which softmax PG methods converge extremely slowly even when perfect model specification is available. Several implications of our result are in order.
% In practice, the policy gradients are typically estimated using samples, and therefore our results also imply the poor sample efficiency of SPG in the worst case. 




\newcommand{\topsepremove}{\aboverulesep = 0mm \belowrulesep = 0mm} \topsepremove


\begin{table}[t]

\begin{center}
	{
\begin{tabular}{c|c|c}
\toprule \hline
%paper & iteration complexity & regularization & learning rates$\vphantom{\frac{1^{7}}{1^{7^3}}}$ \tabularnewline\hline  $\vphantom{\frac{1^{7^{7}}}{1^{7^{7^{7^7}}}}}$
algorithm   &   iteration complexity &  reference    \tabularnewline 
% &  &  &  \tabularnewline	
\hline 
\multirow{2}{*}{PG upper bound} 	 &   \multirow{2}{*}{asymptotic}  & \multirow{2}{*}{\citet[Thm.~5.1]{agarwal2019optimality}}  \tabularnewline
	 &  &      \tabularnewline
\hline 
	\multirow{2}{*}{PG upper bound} 	 &   \multirow{2}{*}{$O \Big( {\color{red}\mathcal{C}^2_{\mathsf{spg}}(\mathcal{M})} \Big\|\frac{d_{\mu}^{\pi^{\star}}}{\mu} \Big\|_{\infty}^2\Big\|\frac{ 1}{\mu} \Big\|_{\infty} \frac{|\cS|}{  (1-\gamma)^2\epsilon} \Big) $}  & \multirow{2}{*}{\citet[Thm.~4]{mei2020global}}  \tabularnewline
	 &  &      \tabularnewline
\hline 
\multirow{2}{*}{NPG upper bound}    &  \multirow{2}{*}{$O\big(\frac{1}{(1-\gamma)^{2}\epsilon}  \big)$  } & \multirow{2}{*}{\citet[Thm.~5.3]{agarwal2019optimality}} \tabularnewline
	 &  &        \tabularnewline
\hline 
	\multirow{2}{*}{PG lower bound}   & \multirow{2}{*}{$ \frac{(1-\gamma)^5 \Delta_{\star}^2}{ 12 \epsilon}   $}   & \multirow{2}{*}{\citet[Thm.~10]{mei2020global}} \tabularnewline
	&  &          \tabularnewline
\hline
	\multirow{2}{*}{PG lower bound} & \multirow{2}{*}{$ |\cS|^{2^{\Omega(\frac{1}{1-\gamma})} } $}   & \multirow{2}{*}{\textbf{this work}} \tabularnewline
	&  &         \tabularnewline
\toprule \hline
\end{tabular}
	}
\end{center}
%
	\caption{Upper and lower bounds on the iteration complexities of PG and NPG methods with softmax parameterization in finding an $\epsilon$-optimal policy obeying $\|V^{\star}-V^{(t)}\|_{\infty}\leq\epsilon \leq 0.15$.  
	% We assume exact policy evaluation and softmax parameterization, and 
	We assume exact gradient evaluation, and hide the dependencies that are logarithmic on problem parameters. Here, $\mu$ denotes the initial state distribution, $\big\|{d_{\mu}^{\pi^{\star}}}/{\mu} \big\|_{\infty}$ is the distribution mismatch coefficient, $a^{\star}(s)$ is the optimal action at state $s$ according to $\pi^{\star}$, $\mathcal{C}_{\mathsf{spg}}(\mathcal{M})\coloneqq  \big( \inf_{s\in \cS }\inf_{t\geq 1} \pi^{(t)}(a^{\star}(s) | s) \big)^{-1}$ is a quantity depending on both the PG trajectory and salient MDP parameters, whereas $\Delta_{\star} : = \min_{s\in \cS, a\neq a^{\star}(s) } \big\{ Q^{\star}(s, a^{\star}(s)) - Q^{\star}(s,a) \big\} $ is the optimality gap of the optimal Q-function $Q^{\star}$.  \label{tab:comparisons}  \vspace{-0.25in}}  
 

\end{table}

\paragraph{Comparisons with prior results.} Table~\ref{tab:comparisons} provides an extensive comparison of the iteration complexities --- including both upper and lower bounds --- of PG and NPG methods under softmax parameterization. As suggested by our result,  the asymptotic iteration complexity $O(1/\epsilon)$ derived in \citet{mei2020global} might not be as rosy as it seems for problems with large state space and long effective horizon; in fact, the crucial quantity $\mathcal{C}_{\mathsf{spg}}(\mathcal{M})$ therein could scale in a prohibitive manner with both $|\cS|$ and $\frac{1}{1-\gamma}$. 
\citet{mei2020global} also developed a lower bound on the iteration complexity of softmax PG methods, which, however, is vacuous (i.e., smaller than $1$) unless $\epsilon$ is very small (e.g., $\epsilon\lesssim (1-\gamma)^3$) for problems with long horizons. 
In addition, \citet{mei2020escaping} provided some evidence that a poorly-initialized softmax PG algorithm can get stuck at suboptimal policies for a single-state MDP (i.e., the bandit problem). This result, however, fell short of providing a complete runtime analysis, and did not capture the influence of a large state space dimension. In contrast, our theory shows that softmax PG can take exponential time to reach even a moderate accuracy regime.

%, while \citet[Section~4.3]{agarwal2019optimality} showed that softmax PG methods could be potentially slow by constructing a chain-like MDP with exceedingly flat saddle points.  
\paragraph{Benchmarking with NPG methods.} Our algorithm-specific lower bound suggests that softmax PG methods --- in their vanilla form --- might take  a pessimistically long time to converge when the state space and effective horizon are large. This is in stark contrast to the convergence rate of NPG methods, 
whose iteration complexity is dimension-free and scales only polynomially in the effective horizon. Consequently, our results shed light on the practical superiority of NPG-based algorithms such as PPO \citep{schulman2017proximal} and TRPO \citep{schulman2015trust}.  


\paragraph{Crux of our design.} As we shall detail momentarily in Section~\ref{sec:mdp-construction}, our exponential lower bound is obtained  through analyzing the trajectory of softmax PG methods on a carefully-designed MDP instance with no more than 3 actions per state, when a uniform initialization scheme and a uniform initial state distribution are adopted. Our construction underscores the critical challenge of {\em credit assignments} \citep{sutton1984temporal} in RL compounded by the presence of delayed rewards, long horizon, and intertwined interactions across states. 


\subsection{Other related work}


%\citet{agarwal2020pc}



\paragraph{Non-asymptotic analysis of (natural) policy gradient methods.} Besides tabular MDPs, finite-time convergence guarantees of PG methods have recently been studied for control problems (e.g., \citet{fazel2018global,jansch2020convergence,tu2019gap,zhang2019policy,mohammadi2019convergence}), MDPs with linear function approximation (e.g., \citet{agarwal2019optimality,cai2019provably}), MDPs with neural network approximation (e.g., \citet{wang2019neural,liu2019neural,agazzi2020global,liu2019neural}), and constrained MDP (e.g., \citet{xu2020primal,ding2020natural}). In addition, non-asymptotic convergence guarantees of NPG methods and their variants have been derived in \citet{agarwal2019optimality,liu2020improved,shani2019adaptive,bhandari2020note,cen2020fast}.

 
 

\paragraph{Other policy parameterizations.} In addition to softmax parameterization, several other policy parameterization schemes have also been investigated in the context of policy optimization and reinforcement learning at large. For example, \citet{agarwal2019optimality,zhang2020variational} studied the converge of projected PG methods with direct parameterization, \citet{asadi2017alternative} introduced the so-called mallow parameterization, while \citet{mei2020escaping} studied the escort parameterization.  Part of these parameterizations were proposed in response to the ineffectiveness of softmax parameterization observed in practice.
 

%\paragraph{Entropy regularization.} Entropy regularization, first proposed in \citet{williams1991function}, has been adopted as a useful strategy to encourage exploration in RL \citep{mnih2016asynchronous,haarnoja2018soft,ahmed2019understanding}. \citet{nachum2017bridging,neu2017unified} explored optimization properties of entropy-regularized RL. \citet{mei2020global} established that SPG with entropy regularization achieves a linear rate of convergence with a pre-constant that depends inversely on the minimum entry of the policy throughout the trajectory of the algorithm, which is unspecified in terms of the dependencies with the MDP parameters. \citet{shani2019adaptive} established a sublinear rate of convergence of NPG with entropy regularization, which is improved by \citet{cen2020fast} to a linear rate that covers soft policy iteration as a special case. 

 
%cite{agarwal2019optimality,fazel2018global,bhandari2019global,mei2020global,cai2019provably,liu2019neural,shani2019adaptive,mei2020global}
 
\paragraph{Lower bounds.} Establishing information-theoretic or algorithmic-specific lower bounds on the statistical and computational complexities of RL algorithms --- often achieved by constructing hard MDP instances --- plays an instrumental role in understanding the bottlenecks of RL algorithms. To give a few examples,
\citet{azar2013minimax} established an information-theoretic lower bound on the sample complexity of learning the optimal policy in a generative model, whereas \citet{khamaru2020temporal,pananjady2020instance} developed instance-dependent lower bounds for policy evaluation. Additionally, \citet{agarwal2019optimality} constructed a chain-like MDP whose value function under direct parameterization  might contain very flat saddle points under a certain initial state distribution, highlighting the role of distribution mismatch coefficients in policy optimization.  Finally, exponential-time convergence of gradient descent has been observed in other nonconvex problems as well (e.g., \citet{du2017gradient}) despite its asymptotic convergence \citep{lee2016gradient}, although the context and analysis therein are drastically different from what happens in RL settings. 

% The recent work \citet{agarwal2019optimality} showed that policy gradient methods, when regularized by the relative entropy (as opposed to  entropy regularization as commonly used in practice and analyzed herein), converges at a rate $O(1/\epsilon^2)$. 
  
  

\paragraph{Notation.}
Denote by $\Delta(\cX)$  the probability simplex over a set $\cX$, and let $|\cS|$ represent the cardinality of the set $\cS$. Many operations should be understood as entry-wise operations when applied to vectors, such as $|\cdot|$,  $\exp(\cdot)$,  $\geq$, $\leq$, and so on. Given two probability distributions $p$ and $q$ over $\cS$, we adopt the notation $\big\| \frac{p}{q} \big\|_{\infty} = \max_{s\in \cS} \frac{p(s)}{q(s)}$ and $\big\| \frac{1}{q} \big\|_{\infty} = \max_{s\in \cS} \frac{1}{q(s)}$ .

%The softmax function $\mathsf{softmax}: \mathbb{R}^n \mapsto \mathbb{R}^n$ is defined such that $ [\mathsf{softmax}(\theta) ]_i :=  \exp(\theta_i) / \big( \sum_{i} \exp(\theta_i)  \big) $ for a vector $\theta=[\theta_i]_{1\leq i\leq n}\in \mathbb{R}^n$, where

%For any vectors $z=[z_i]_{1\leq i\leq n}$ and $w=[w_i]_{1\leq i\leq n}$, the notation $z \geq w$ (resp.~$ z \leq  w$) means $z_i \geq w_i$ (resp.~$z_i\leq w_i$) for all $1\leq i\leq n$. 

%When scalar functions such as $|\cdot|$, $\exp(\cdot)$ and $\log(\cdot)$ are applied to vectors, their applications should be understood in an entry-wise fashion. 
%For instance, given any vector $z=[z_i]_{1\leq i\leq n}\in \mathbb{R}^n$, the notation $|\cdot|$ denotes $|z|:=[|z_i|]_{1\leq i\leq n}$; other functions are defined analogously. 



==> monotone-lemma.tex <==
%\section{Preliminaries: monotonicity of value estimates}
%
%
%
%
%\paragraph{Unregularized policy gradient methods.} 
%
%Akin to  standard monotonicity properties of gradient descent \citep{beck2017first}, the unregularized PG update is known to achieve monotonic performance improvement, as formally stated below. The interested reader is referred to \citet[Lemma C.2]{agarwal2019optimality} for the proof.
%%
%\begin{lemma}
%	\label{lem:ascent-lemma-PG}
%	Consider the policy gradient update rule \eqref{eq:PG-update-all} without entropy regularization (i.e., $\lambda=0$). If $0<\eta< (1-\gamma)^2 / 5$, then for any $t\geq 0$ one has
%	%
%	\begin{align*}
%		\forall (s,a)\in \cS\times \cA: \qquad V^{(t+1)}(s) \geq V^{(t)}(s)
%		\qquad \text{and}\qquad 
%		Q^{(t+1)}(s,a) \geq Q^{(t)}(s,a).
%	\end{align*}
%	%
%\end{lemma}
%%
%This monotonicity feature, in conjunction with the uniform initialization scheme, ensures non-negativity of value function estimates throughout the execution of the algorithm.
%%
%\begin{lemma}
%	\label{lem:non-negativity-PG}
%	Consider the unregularized policy gradient update rule \eqref{eq:PG-update-all} with $\lambda = 0$, and suppose the initial policy $\pi^{(0)}(\cdot \mymid s)$ for any $s\in \cS$ is given by a uniform distribution over the action space. Then one has
%	%
%	\begin{align*}
%		\forall t\geq 0, ~ \forall s\in \cS: \qquad  V^{(t)}(s) \geq 0.
%	\end{align*}
%	%
%\end{lemma}
%%
%\begin{proof}
%	Recall that the only negative rewards in our constructed MDP are $r(s_1,a_0)$ for $s_1\in \cS_1$ and $r(s_2,a_0)$ for $s_2\in \cS_2$. When $\pi^{(0)}(\cdot\mymid s_1)$ is uniformly distributed, the MDP specification \eqref{eq:P-r-state-S1S2} gives
%	\[
%		\forall s_1\in \cS_1: \qquad V^{(0)}(s_1) = 0.5 r(s_1,a_0) + 0.5 r(s_1,a_1) = 0.
%	\]
%	%
%	Similarly, one has $V^{(0)}(s_2)=0$ for all $s_2\in \cS_2$. From the Bellman equation, it is easily seen that the  value function $V^{(0)}$ of any other state is a linear combination of $\{r(s,a)\mymid s\notin \cS_1, s\notin \cS_2\}$, $\{V^{(0)}(s_1) \mymid s_1\in \cS_1 \}$ and $\{V^{(0)}(s_2)\mymid s_2\in \cS_2\}$, which are all non-negative. It thus follows that the initial estimates $V^{(0)}(s)\geq 0$ for all $s\in \cS$. Apply Lemma~\ref{lem:non-negativity-PG} to conclude that $V^{(t)}(s)\geq V^{(0)}(s) \geq 0$ for any $s\in \cS$ and any $t\geq 0$.
%\end{proof}
%
%
%
%\paragraph{Entropy-regularized policy gradient methods.} 
%
%The situation becomes more complicated when we turn attention to entropy-regularized PG methods. 
%Given that gradient ascent is applied w.r.t.~the {\em regularized} value function,  in general one cannot ensure the {\em unregularized} value estimates to be monotonically increasing over time. Fortunately, by imposing additional assumptions, one can guarantee that the gradient of the regularization term is entrywise dominated by that of the original value function, thereby allowing for monotonicity in terms of the unregularized value function. This constitutes one of our key findings to be presented in this section.  
%
%We have
%\begin{itemize}
%\item $\Ent^{(t)}(0) = 0$, and $\soft{V}^{(t)}(0) = V^{(t)}(0) = 0$.
%\item For all $s \in \cS_1 \cup \cS_2$ and $a \in \cA_s$,
%\[
%\soft{Q}^{(t)}(s, a) = Q^{(t)}(s, a) - \lambda \log \pi^{(t)}(a|s).
%\]
%\item For all $1 \le s \le H$,
%\[
%\soft{Q}^{(t)}(\overline{s}, a_0) = Q^{(t)}(\overline{s}, a_0) - \lambda \log \pi^{(t)}(a_0|\overline{s}),
%\]
%and
%\[
%\soft{Q}^{(t)}(\overline{s}, a_1) = Q^{(t)}(\overline{s}, a_1) - \lambda \log \pi^{(t)}(a_1|\overline{s}) + \gamma\lambda \Ent^{(t)}(s).
%\]
%\item For all $3 \le s \le H$,
%\[
%\soft{Q}^{(t)}(s, a_0) = Q^{(t)}(s, a_0) - \lambda \log \pi^{(t)}(a_0|s),
%\]
%\[
%\soft{Q}^{(t)}(s, a_1) = Q^{(t)}(s, a_1) - \lambda \log \pi^{(t)}(a_1|s) + \gamma\lambda \Ent^{(t)}(\overline{s-1}),
%\]
%and 
%\[
%\soft{Q}^{(t)}(s, a_2) = Q^{(t)}(s, a_2) - \lambda \log \pi^{(t)}(a_2|s) + \gamma p \lambda \Ent^{(t)}(\overline{s-2}).
%\]
%\item It can be shown that for any $t \ge 0$ and $s \in \cS$,
%\begin{align*}
%\Ent^{(t)}(s) \le 4,
%\end{align*}
%and then
%\begin{align}
%\lambda \Ent^{(t)}(s) \le c_{\lambda}(1-\gamma).
%\end{align}
%As a consequence, for any $s \in \cS_1 \cup \cS_2 \cup \{3, 4, \ldots, H\} \cup \{\overline{1}, \overline{2}, \ldots, \overline{H}\}$ and any $t \geq 0$,
%\[
%|\soft{A}^{(t)}(s, a) - \widehat{A}^{(t)}(s, a)| \le c_{\lambda}(1-\gamma)(1-\pi^{(t)}(a|s)),
%\]
%where $\widehat{A}^{(t)}(s, a) \defn A^{(t)}(s, a) - \lambda\Big(\theta^{(t)}(s, a) - \sum_{a^{\prime}} \pi^{(t)}(a^{\prime}\mymid s)\theta^{(t)}(s, a)\Big)$.
%\end{itemize}
%
%
%\begin{lemma} \label{lem:entropy-bound}
%Suppose that $\pi^{(t)}(a_1|s^{\prime}), \pi^{(t)}(a_1|\overline{s^{\prime}}) > 1-(1-\gamma)^2/64$ holds for any $s^{\prime} < s$, if $\pi^{(t)}(a_1|s) > 1/2$.
%Then, for any $s \in \cS_1 \cup \cS_2 \cup \{3, 4, \ldots, H\} \cup \{\overline{1}, \overline{2}, \ldots, \overline{H}\}$ and any $t \geq 0$,
%\begin{align}
%\Ent^{(t)}(s) \le 4.
%\end{align}
%\end{lemma}
%
%\begin{proof}
%The entropy enjoys the following version of Bellman equation,
%\begin{align}
%\Ent^{(t)}(s) = -\sum_{a \in \cA_s}\pi^{(t)}(a|s)\log\pi^{(t)}(a|s) + \gamma\sum_{s^{\prime}} P(s^{\prime} \mymid s, \pi^{(t)})\Ent^{(t)}(s^{\prime}).
%\end{align}
%Since $|\cA_0| = 1$ and $P(0 \mymid 0, a_0) = 1$, we have $\Ent^{(t)}(0) = 0$, and then for any $s \in \cS_1 \cup \cS_2$, $\Ent^{(t)}(s) = -\sum_{a \in \cA_s}\pi^{(t)}(a|s)\log\pi^{(t)}(a|s) \le \log 2$.
%In addition, for any $s \in \{\overline{1}, \overline{2}, \ldots, \overline{H}\}$
%\begin{align*}
%\Ent^{(t)}(\overline{s}) = -\sum_{a \in \cA_{\overline{s}}}\pi^{(t)}(a|\overline{s})\log\pi^{(t)}(a|\overline{s}) + \gamma \pi^{(t)}(a_1|\overline{s})\Ent^{(t)}(s),
%\end{align*}
%and for any $s \in \{3, 4, \ldots, H\}$
%\begin{align*}
%\Ent^{(t)}(s) = -\sum_{a \in \cA_{s}}\pi^{(t)}(a|s)\log\pi^{(t)}(a|s) + \gamma \pi^{(t)}(a_1|s)\Ent^{(t)}(\overline{s-1}) + \gamma p \pi^{(t)}(a_2|s)\Ent^{(t)}(\overline{s-2}).
%\end{align*}
%With these relations in hand, we will show, by induction method, $\Ent^{(t)}(s) \le \Ent_{\mathsf{max}} \defn \log 18$ and then $\Ent^{(t)}(\overline{s}) \le \overline{\Ent}_{\mathsf{max}} \le \log 2 + \Ent_{\mathsf{max}}$.
%If $\pi^{(t)}(a_1|s^{\prime}) \le \frac{1}{2}$, we have
%\begin{align*}
%\Ent^{(t)}(s) \le \log 3 + \gamma (\frac{1}{2}+p) \overline{\Ent}_{\mathsf{max}} \le \Ent_{\mathsf{max}}.
%\end{align*}
%Otherwise, for any $s^{\prime} < s$, we have $-\sum_{a \in \cA_{s^{\prime}}}\pi^{(t)}(a|s^{\prime})\log\pi^{(t)}(a|s^{\prime}) \le 1-\gamma$ and $-\sum_{a \in \cA_{\overline{s^{\prime}}}}\pi^{(t)}(a|\overline{s^{\prime}})\log\pi^{(t)}(a|\overline{s^{\prime}}) \le 1-\gamma$, which gives $\Ent^{(t)}(s^{\prime}) \le 1$, and $\Ent^{(t)}(\overline{s^{\prime}}) \le 1$.
%Hence,
%\begin{align*}
%\Ent^{(t)}(s) \le \log 3 + \gamma \le \Ent_{\mathsf{max}}.
%\end{align*}
%Then, we conclude the proof here.
%\end{proof}
%
%
%\begin{lemma} 
%	\label{lem:theta-t}
%For any $s \in \cS_1 \cup \cS_2 \cup \{3, 4, \ldots, H\} \cup \{\overline{1}, \overline{2}, \ldots, \overline{H}\}$ and any $t \geq 0$, it follows that
%%
%\begin{align}
%	|\theta^{(t)}(s, a)| \le 6\log (t+1) + 3,
%\end{align}
%%
%provided that $0\leq \lambda \le 1/3$ and $0< \eta \le (1-\gamma)/3$.
%\end{lemma}
%
%
%
%\begin{lemma}
%\label{lem:Vlambda-V-equiv}
%Suppose that 
%%
%\begin{equation}
%\frac{\partial V_{\lambda}^{\pi_{\bmtheta}}(\mu)}{\partial\theta(s,a)}=c_{\nu}\frac{\partial V^{\pi_{\bmtheta}}(\mu)}{\partial\theta(s,a)},\qquad\text{for some }c_{\nu}\in\left[\frac{1}{3},2\right].\label{eq:Vlambda-V-equiv}
%\end{equation}
%%
%\end{lemma}
%%
%\begin{proof}
%Recall that
%%
%\begin{align*}
%\frac{\partial V_{\lambda}^{\pi_{\theta}}(\mu)}{\partial\theta(s,a)} & =\frac{1}{1-\gamma}d_{\mu}^{\pi_{\theta}}(s)\pi_{\theta}(a\mymid s)\Big\{ Q^{\pi_{\theta}}(s,a)-V^{\pi_{\theta}}(s)-\lambda\theta(s,a)+\lambda\sum_{a'}\pi_{\theta}(a'\mymid s)\,\theta(s,a')\Big\}\\
% & =\frac{1}{1-\gamma}d_{\mu}^{\pi_{\theta}}(s)\pi_{\theta}(a\mymid s)\Big\{\sum_{a':a'\neq a}\pi_{\theta}(a'\mymid s)\Big[Q^{\pi_{\theta}}(s,a)-Q^{\pi_{\theta}}(s,a')\Big]-\lambda\sum_{a':a'\neq a}\pi_{\theta}(a'\mymid s)\,\Big[\theta(s,a)-\theta(s,a')\Big]\Big\}.
%\end{align*}
%%
%As an implication, if 
%
%
%\end{proof}
%
%
%Based on the above two lemmas, for all $t \le \exp(\frac{c}{\varepsilon})$, where $c > 0$ is some constant, we have 
%\begin{align*}
%\lambda |\theta(s, a)| \le&~(e+1)(1-\gamma)\varepsilon \cdot 2\log t \\
%\le&~2c(e+1)(1-\gamma).
%\end{align*}
%Hence, in the following, we assume that $\lambda |\theta(s, a)| \leq c_{\lambda}(1-\gamma)$ for some small constant $c_{\lambda} = 2c(e+1) > 0$.
%Then we have for some constant $\frac{1}{3} \leq c \leq 2$, 
%\begin{align*}
%\frac{\partial V^{\pi_{\bmtheta}}(\mu) + \lambda \Ent^{\pi_{\bmtheta}}_{\mu}(\pi_{\bmtheta})}{\partial \theta(s, a)} = c\frac{\partial V^{\pi_{\bmtheta}}(\mu)}{\partial \theta(s, a)},
%\end{align*}
%provided that 
%\begin{align} \label{eq:equiv-cond}
%|Q^{\pi_{\bmtheta}}(s, a) - V^{\pi_{\bmtheta}}(s)| = \big|\sum_{a^{\prime} \ne a} \pi_{\bmtheta}(a^{\prime}|s)(Q^{\pi_{\bmtheta}}(s, a) - Q^{\pi_{\bmtheta}}(s, a^{\prime}))\big| \geq 3c_{\lambda}(1-\gamma)(1-\pi_{\bmtheta}(a|s)).
%\end{align}
%In addition, let $\tau^{+} \defn \tau + 4c_{\lambda}(1-\gamma)$ and $\tau^{-} \defn \tau - 4c_{\lambda}(1-\gamma)$ for any constant $\tau > 0$.
%
%\begin{lemma}
%	\label{lem:ascent-lemma-entropy}
%	Consider the policy gradient update rule with entropy regularization. For $3 \leq s \leq H$ one has if $V^{(t)}(s) \geq \tau_s^{-}$,
%	%
%	\begin{align*}
%		\forall a\in \cA: \qquad V^{(t+1)}(s) \geq V^{(t)}(s),\qquad \text{and}\qquad Q^{(t+1)}(s,a) \geq Q^{(t)}(s,a).
%	\end{align*}
%	%
%	Moreover, for any $t\geq 0$ and any state $s \in \cS_1 \cup \cS_2$,
%	\begin{align*}
%	V^{(t+1)}(s) \geq V^{(t)}(s).
%	\end{align*}
%	For $1 \leq s \leq H$ and $V^{(t)}(s) \geq \tau_s^{+}$,
%	\begin{align*}
%	V^{(t+1)}(\overline{s}) \geq V^{(t)}(\overline{s}).
%	\end{align*}
%\end{lemma}
%
%
%
%
%
%\begin{lemma}
%	\label{lem:non-negativity-PG-entropy}
%	Consider the policy gradient update rule \eqref{eq:PG-update-all}, and suppose that the initial policy $\pi^{(0)}(\cdot \mymid s)$ for any $s\in \cS$ is given by a uniform distribution over the associated action space. Then one has
%	%
%	\begin{align*}
%		\forall t\geq 0, ~ \forall s\in \cS: \qquad  V^{(t)}(s) \geq 0.
%	\end{align*}
%	%
%\end{lemma}
%%
%\begin{proof}
%	The only negative rewards in our constructed MDP are $r(s_1,a_0)$ for $s_1\in \cS_1$ and $r(s_2,a_0)$ for $s_2\in \cS_2$. When $\pi^{(0)}(\cdot\mymid s_1)$ is uniformly distributed, the MDP specification \eqref{eq:P-r-state-S1S2} gives
%	\[
%		\forall s_1\in \cS_1: \qquad V^{(0)}(s_1) = 0.5 r(s_1,a_0) + 0.5 r(s_1,a_1) = 0.
%	\]
%	%
%	Similarly, one has $V^{(0)}(s_2)=0$ for all $s_2\in \cS_2$. From the Bellman equation, it is easily seen that the  value function $V^{(0)}$ of any other state is a linear combination of $\{r(s,a)\mymid s\notin \cS_1, s\notin \cS_2\}$, $\{V^{(0)}(s_1) \mymid s_1\in \cS_1 \}$ and $\{V^{(0)}(s_2)\mymid s_2\in \cS_2\}$, which are all non-negative. It thus follows that $V^{(0)}(s)\geq 0$ for any $s\in \cS$. Apply Lemma~\ref{lem:non-negativity-PG} to conclude that $V^{(t)}(s)\geq V^{(0)}(s) \geq 0$ for any $s\in \cS$ and any $t\geq 0$.
%\end{proof}
%
%
%\begin{lemma}
%	\label{lem:ascent-lemma-softV}
%	Consider the policy gradient update rule with entropy regularization. For any $s \in \cS_1 \cup \cS_2 \cup \{3, 4, \ldots, H\} \cup \{\overline{1}, \overline{2}, \ldots, \overline{H}\}$ and any $t \geq 0$, it follows that
%%
%\begin{align}
%	\soft{V}^{(t+1)}(s) \ge \soft{V}^{(t)}(s),
%\end{align}
%%
%provided that $0\leq \lambda \le 1/3$ and $0< \eta \le (1-\gamma)/10$.
%\end{lemma}
%
%\begin{proof}
%This lemma can be proved by showing that:
%if for any state $s^{\prime}$ satisfying that there exists some action $a$ with $P(s^{\prime}|s, a) > 0$, $\soft{V}^{(t+1)}(s^{\prime}) \ge \soft{V}^{(t)}(s^{\prime})$, then we have
%\[
%\soft{V}^{(t+1)}(s) \ge \soft{V}^{(t)}(s).
%\]
%Since
%\begin{align*}
%\soft{V}^{(t+1)}(s) =&~\sum_a \pi^{(t+1)}(a|s)\soft{Q}^{(t+1)}(s, a) \\
%=&~\sum_a \pi^{(t+1)}(a|s)(\soft{r}^{(t+1)}(s, a)+\gamma\sum_{s^{\prime}}P(s^{\prime}|s, a)\soft{V}^{(t+1)}(s^{\prime})) \\
%\ge&~\sum_a \pi^{(t+1)}(a|s)(r(s, a)-\lambda\log\pi^{(t+1)}(a|s)+\gamma\sum_{s^{\prime}}P(s^{\prime}|s, a)\soft{V}^{(t)}(s^{\prime})),
%\end{align*}
%then it is sufficient to show
%\[
%\sum_a \pi^{(t+1)}(a|s)(c(s, a)-\lambda\log\pi^{(t+1)}(a|s)) \ge \soft{V}^{(t)}(s) = \sum_a \pi^{(t)}(a|s)(c(s, a)-\lambda\log\pi^{(t)}(a|s)),
%\]
%which follows from the smoothness of $F(\theta) \defn \sum_a \pi_{\theta}(a|s)(c(s, a)-\lambda\log\pi_{\theta}(a|s))$ with $|c(s, a)| < 2$.
%\end{proof}
%
%
%
%\subsection{Proof of Lemma~\ref{lem:ascent-lemma-entropy}}
%We prove this lemma by dividing it into two cases.
%\begin{itemize}
%\item \textbf{Case I:} $|\cA| = 2$. For $s \in \cS_1 \cup \cS_2$, we have
%\[
%Q^{\pi_{\bmtheta}}(s, a_1) - Q^{\pi_{\bmtheta}}(s, a_0) \geq 3c_{\lambda}(1-\gamma).
%\]
%Then, we know that $\theta(s, a_1)$ is increasing since
%\[
%\frac{\partial V^{\pi_{\bmtheta}}(\mu) + \lambda \Ent^{\pi_{\bmtheta}}_{\mu}(\pi_{\bmtheta})}{\partial \theta(s, a)} \asymp \frac{\partial V^{\pi_{\bmtheta}}(\mu)}{\partial \theta(s, a)} > 0,
%\]
%while $\theta(s, a_0)$ is decreasing.
%Hence, the monotonicity is obvious.
%For $1 \leq s \leq H$ and $V^{(t)}(s) \geq \tau_s + 4c_{\lambda}(1-\gamma)$,
%\[
%Q^{(t)}(\overline{s}, a_1) - Q^{(t)}(\overline{s}, a_0) \geq 3c_{\lambda}(1-\gamma).
%\]
%Similarly, we know that $\theta(s, a_1)$ is increasing and $\theta(s, a_0)$ is decreasing.
%In addition, $V^{(t)}(s)$ is also increasing due to the claim, which gives that $Q^{(t+1)}(\overline{s}, a_1) = \gamma V^{(t+1)}(s) \ge Q^{(t)}(\overline{s}, a_1)$.
%Then, we prove the claim for $\overline{s}$.
%\item \textbf{Case II:} $|\cA| = 3$. Notice that $V^{(t)}(s) \geq \tau_s - 4c_{\lambda}(1-\gamma)$ means that $V^{(t)}(\overline{s-1}) \geq \gamma\tau_{s-1} + 4c_{\lambda}(1-\gamma)$, and then $Q^{(t+1)}(s, a) \ge Q^{(t)}(s, a)$.
%Notice that $Q^{(t)}(s, a_1) - \max\{Q^{(t)}(s, a_0), Q^{(t)}(s, a_2)\} \geq 3c_{\lambda}(1-\gamma)$, and $V^{(t)}(s) - \max\{Q^{(t)}(s, a_0), Q^{(t)}(s, a_2)\} \geq 3c_{\lambda}(1-\gamma)$.
%Hence, we have $\theta^{(t+1)}(s, a) \ge \theta^{(t)}(s, a)$ if and only if $A^{(t)}(s, a) \ge 0$.
%Then,
%\begin{align*}
%V^{(t+1)}(s) - V^{(t)}(s) =&~\sum_a \pi^{(t+1)}(a|s)Q^{(t+1)}(s, a) - V^{(t)}(s) \\
%\ge&~\sum_a \pi^{(t+1)}(a|s)A^{(t)}(s, a) \\
%=&~\frac{\sum_a \exp(\theta^{(t+1)}(s, a))A^{(t)}(s, a)}{\sum_a \exp(\theta^{(t+1)}(s, a))} \\
%\ge&~\frac{\sum_a \exp(\theta^{(t)}(s, a))A^{(t)}(s, a)}{\sum_a \exp(\theta^{(t+1)}(s, a))} = 0.
%\end{align*}
%\end{itemize}
%
%
%
%
%
%
%\subsection{Proof of Lemma~\ref{lem:theta-t}}
%%
%Consider any parameter $\theta = [\theta(s,a)]$ obeying $\sum_a\theta(s,a)=0$ for all $s\in \cS$.  Let us define
%%
%\begin{align*}
%	\theta_{\mathsf{max}}(s) \defn \max_a \theta(s, a), 
%	\quad  
%	\theta_{\mathsf{min}}(s) \defn \min_a \theta(s, a), 
%	\quad \text{and} \quad 
%	\theta_{\mathsf{gap}}(s) \defn \theta_{\mathsf{max}}(s) - \theta_{\mathsf{min}}(s),
%\end{align*}
%%
%which clearly satisfies $\theta_{\mathsf{max}}(s) \geq 0$ and $\theta_{\mathsf{min}}(s)\leq 0$. 
%When  $|\cA_s| = 3$, it is seen that
%%
%\[
%\begin{cases}
%0 & =\sum_{a}\theta(s,a)\leq\theta_{\mathsf{min}}(s)+2\theta_{\mathsf{max}}(s),\\
%0 & =\sum_{a}\theta(s,a)\geq2\theta_{\mathsf{min}}(s)+\theta_{\mathsf{max}}(s),
%\end{cases}\qquad\Longrightarrow\qquad\begin{array}{cc}
%	& - 0.5 \theta_{\mathsf{min}}(s)  \leq\theta_{\mathsf{max}}(s)\leq-2\theta_{\mathsf{min}}(s).\\
% & \theta_{\mathsf{gap}}(s)\leq-3\theta_{\mathsf{min}}(s).
%\end{array}
%\]
%%
%Similarly, when $|\cA_s| = 2$ one has
%%
%\[
%0=\theta_{\mathsf{min}}(s)+\theta_{\mathsf{max}}(s),\qquad\Longrightarrow\qquad\begin{array}{cc}
% & \theta_{\mathsf{max}}(s)=-\theta_{\mathsf{min}}(s).\\
% & \theta_{\mathsf{gap}}(s)=-2\theta_{\mathsf{min}}(s).
%\end{array}
%\]
%%
%To summarize, in both cases we have
%%
%\begin{align}
%	-0.5\theta_{\mathsf{min}}(s) \leq \theta_{\mathsf{max}}(s)\leq-3\theta_{\mathsf{min}}(s)\qquad\text{and}\qquad\theta_{\mathsf{gap}}(s)\leq-3\theta_{\mathsf{min}}(s).
%	\label{eq:theta-max-gap-range-min}
%\end{align}
%%
%Given that $\pi(a\mymid s)$ is proportional to $\theta(s,a)$,  an immediate consequence of the preceding inequalities is that
%%
%\[
%\min_{a}\pi(a\mymid s)=\frac{\exp\big(\theta_{\mathsf{min}}(s)\big)}{\sum_{a}\exp\big(\theta(s,a)\big)}\leq\frac{\exp\big(\theta_{\mathsf{min}}(s)\big)}{\exp\big(\theta_{\mathsf{max}}(s)\big)}\leq\frac{\exp\big(\theta_{\mathsf{min}}(s)\big)}{\exp\big(-0.5\theta_{\mathsf{min}}(s)\big)}=\exp\big(1.5\theta_{\mathsf{min}}(s)\big).
%\]
%%
%Additionally, the gradient of the regularized value function satisfies
%%
%\begin{align*}
%	\left|\frac{\partial V_{\lambda}^{\pi_{\bmtheta}}(\mu) }{\partial \theta(s, a)}\right| 
%	\le \frac{1}{1-\gamma} \pi_{\bmtheta}(a|s) \big( 2+\lambda \theta_{\mathsf{gap}}(s) \big) 
%	\leq \frac{1}{1-\gamma} \pi_{\bmtheta}(a|s) \big( 2- \theta_{\mathsf{min}}(s) \big) ,
%\end{align*}
%%
%where the first inequality makes use of the facts $d^{\pi_{\bmtheta}}_{\mu}(s) \le 1$
%	and $|Q^{\pi_{\bmtheta}}(s, a) - V^{\pi_{\bmtheta}}(s)| \le \max_{s,a}|Q^{\pi_{\bmtheta}}(s, a)| +\max_s |V^{\pi_{\bmtheta}}(s)| \leq 2$ (in view of Lemma \ref{lem:basic-properties-MDP-Vstar}), and the last one follows since  $\theta_{\mathsf{gap}}(s)\leq-3\theta_{\mathsf{min}}(s)$ and $\lambda \leq 1/3$. 
%
%
%With the above basic properties in mind, if we set $\theta_{\mathsf{min}}^{(t+1)}(s)\defn \min_a \theta^{(t)}(s,a)$ and  $a_{\mathsf{min}}^{(t)}=\arg\min_a \theta^{(t)}(s,a)$, 
%then the PG update rule gives
%%
%\begin{align}
%\theta_{\mathsf{min}}^{(t+1)}(s) & \geq\theta^{(t)}\big(s,a_{\mathsf{min}}^{(t)}\big)-\eta\left|\frac{\partial V_{\lambda}^{(t)}(\mu)}{\partial\theta\big(s,a_{\mathsf{min}}^{(t)}\big)}\right|\geq\theta^{(t)}\big(s,a_{\mathsf{min}}^{(t)}\big)-\frac{\eta}{1-\gamma}\pi\big(a_{\mathsf{min}}^{(t)}\mymid s\big)\big(2-\theta_{\mathsf{min}}^{(t)}(s)\big) \notag\\
% & \ge\theta_{\mathsf{min}}^{(t)}(s)-\frac{\eta}{1-\gamma}\exp\big(1.5\theta_{\mathsf{min}}^{(t)}(s)\big)\big(2-\theta_{\mathsf{min}}^{(t)}(s)\big) \notag\\
%	& \ge\theta_{\mathsf{min}}^{(t)}(s)-\frac{1}{3}\exp\big(1.5\theta_{\mathsf{min}}^{(t)}(s)\big)\big(2-\theta_{\mathsf{min}}^{(t)}(s)\big),
%	\label{eq:theta-t-recursion-min}
%\end{align}
%%
%where the last inequality is valid when $0<\eta \leq (1-\gamma) / 3$. 
%
%
%It then boils down to controlling $\theta_{\mathsf{min}}^{(t)}(s)$ on the basis of \eqref{eq:theta-t-recursion-min}.  
%Given that $\theta_{\mathsf{min}}^{(t)}(s)\leq 0$ for all $t\geq 0$, it suffices to study the following non-negative sequence $\{b_t\}_{t\geq 0}$ obeying
%%
%\begin{align}
%	0\leq b_{t+1}\leq b_{t}+  \frac{2+b_{t}}{3\exp(1.5b_{t})} .
%	\label{eq:theta-t-recursion-bt}
%\end{align}
%%
%We claim that this sequence obeys $$b_t \leq 2\log (t+1) + 1  \qquad \text{for all } t\geq 0,$$ which we shall establish by induction. 
%To begin with, for the base case with $t=0$,  we have $b_t=0$, which clearly satisfies the induction hypothesis. 
%Now, suppose that $b_t \leq 2\log (t+1) + 1$ holds for the $t$-th iteration, and we would like to bound $b_{t+1}$. Towards this, we divide into two cases. 
%First of all, if $0\leq b_{t}\leq\frac{4}{3}\log t$, then the above relation \eqref{eq:theta-t-recursion-bt} implies that 
%%
%\[
%	b_{t+1}\leq b_{t}+\frac{1}{3}\frac{2+b_{t}}{\exp(1.5b_{t})}\leq\frac{4}{3}b_{t}+\frac{2}{3}\leq\frac{16}{9}\log t +\frac{2}{3}<2\log(t+2)+1.
%\]
%%
%Otherwise, if instead $\frac{4}{3}\log t\leq b_{t}\leq2\log (t+1) +1$ holds, then it is readily seen that 
%%
%\[
%	b_{t+1}\leq b_{t}+\frac{1}{3}\frac{2+b_{t}}{\exp(1.5b_{t})}\leq2\log (t+1) +\frac{3+2\log (t+1) }{3t^{2}}+1\leq2\log(t+2)+1,
%\]
%%
%where the last inequality is an elementary fact that holds for any $t\geq0$. 
%This in turn justifies that $b_{t+1}\leq \log(t+2) + 1$, thus establishing the claimed upper bound on $b_t$. 
%As a consequence, we can conclude that 
%%
%\[
%	0\geq \theta_{\mathsf{min}}^{(t)}(s) \geq -2\log (t+1) -1 \qquad \text{for all }t\geq 0 .
%\]
%%
%Putting this result together with  \eqref{eq:theta-max-gap-range-min} yields $0\leq \theta_{\mathsf{min}}^{(t)}(s) \leq 6\log (t+1) +3$ for all $t\geq 0$.
%These taken collectively conclude the proof. 
%%
%
%%which gives that, if $\theta_{\mathsf{min}}^{(t)}(s) \ge -\log t$, $\theta_{\mathsf{min}}^{(t+1)}(s) \ge -\log(t+1)$. Hence the lemma is concluded.
%
%
%

